Raw Text is All you Need: Knowledge-intensive Multi-turn Instruction Tuning for Large Language Model

Instruction tuning as an effective technique aligns the outputs of large language models (LLMs) with human preference. But how to generate the seasonal multi-turn dialogues from raw documents for instruction tuning still requires further exploration. In this paper, we present a novel framework named R2S that leverages the CoD-Chain of Dialogue logic to guide large language models (LLMs) in generating knowledge-intensive multi-turn dialogues for instruction tuning. By integrating raw documents from both open-source datasets and domain-specific web-crawled documents into a benchmark K-BENCH, we cover diverse areas such as Wikipedia (English), Science (Chinese), and Artifacts (Chinese). Our approach first decides the logic flow of the current dialogue and then prompts LLMs to produce key phrases for sourcing relevant response content. This methodology enables the creation of the G I NSTRUCT instruction dataset, retaining raw document knowledge within dialoguestyle interactions. Utilizing this dataset, we fine-tune GLLM, a model designed to transform raw documents into structured multi-turn dialogues, thereby injecting comprehensive domain knowledge into the SFT model for enhanced instruction tuning. This work signifies a stride towards refining the adaptability and effectiveness of LLMs in processing and generating more accurate, contextually nuanced responses across various fields.

==> Tables/case_study_single_column.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{3mm}        % 控制列间距
% \begin{tabular}{m{7cm}}
% \toprule
% \textbf{Title} \\
% 2006-2007: Ciara: The Evolution and acting debut                                   \\ \midrule
% \textbf{Document} \\ 
%   On December 5, 2006, Ciara released her second studio album, Ciara: The Evolution. According to the singer, the title of the album is \textbackslash{}"about so much more than just my personal growth - it's about the evolution of music, the evolution of dance, the evolution of fashion \textbackslash{}"\dots \\ \midrule
% \textbf{Dialogue} \\  Usr:\begin{tabular}{m{6.0cm}}What was the evolution?\end{tabular}                                         \\ \cmidrule(l){1-1} 
%                             Sys:\begin{tabular}{m{6.0cm}}On December 5, 2006, Ciara released her second studio album, Ciara: The Evolution.\end{tabular} \\ \cmidrule(l){1-1} 
%                             Usr:\begin{tabular}{m{6.0cm}}What was the name of the album?\end{tabular}                                                    \\ \cmidrule(l){1-1} 
%   Sys:\begin{tabular}{m{6.0cm}}The title of the album is \textbackslash{}"about so much more than just my personal growth - it's about the evolution of music, the evolution of dance, the evolution of fashion.\textbackslash{}"\end{tabular} \\ \cmidrule(l){1-1}  \dots \\ \bottomrule
% \end{tabular}
% \caption{An example of the synthetic conversation generated by AutoConv, the LLM is finetuned with 50 human dialogues from QuAC \cite{DBLP:conf/emnlp/ChoiHIYYCLZ18}.}
% \label{tab:case_study_single_column}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{0mm}        % 控制列间距
\renewcommand{\arraystretch}{1.15}  % 控制行高
\begin{tabular}{m{15cm}}  % 控制宽度
% \toprule
\noalign{\hrule height 1.5pt} % 控制上下线粗细
% \rowcolor{ggray!20}
\multicolumn{1}{c}{\textbf{Reference}} \\
\hline
Beyoncé.A self-described \"modern-day feminist\", Beyonc creates songs that are often characterized by themes of love, relationships, and monogamy, as well as female sexuality and empowerment. On stage, her dynamic, highly choreographed performances have led to critics hailing her as one of the best entertainers in contemporary popular music. Throughout a career spanning 19 years, she has sold over 118 million records as a solo artist, and a further 60 million with Destiny's Child, making her one of the best-selling music artists of all time. \dots \\ 
% She has won 20 Grammy Awards and is the most nominated woman in the award's history. The Recording Industry Association of America recognized her as the Top Certified Artist in America during the 2000s decade. In 2009, Billboard named her the Top Radio Songs Artist of the Decade, the Top Female Artist of the 2000s and their Artist of the Millennium in 2011. Time listed her among the 100 most influential people in the world in 2013 and 2014. Forbes magazine also listed her as the most powerful female musician of 2015.

% \rowcolor{ggray!20}
\hline
\multicolumn{1}{c}{\textbf{Role}} \\ 
\hline
  base:[A: Beyoncé, modern-day feminist] [B: Critic] \\
  my:[A: Music Enthusiast  B: Music Critic] \\

% \rowcolor{ggray!20}
\hline
\multicolumn{1}{c}{\textbf{Dialogue}} \\ 
\hline
\textbf{Base} \\ 
"A": "I admire Beyoncé's empowering songs and performances.", \\ 
"B": "Indeed, she's a modern-day feminist icon in the music industry." \\ 
"A": "Her record sales and Grammy wins are truly impressive.", \\ 
"B": "Yes, she's one of the best-selling and most awarded artists." \\ 
"A": "Beyoncé's influence extends beyond music. She's on Time's influential list.", \\ 
"B": "She's not just a singer but a cultural icon shaping society." \\ 
"A": "Forbes recognized her as the most powerful female musician in 2015.", \\ 
"B": "That's a testament to her impact and success in the industry." \\ 
\dots \\
% "A": "Do you think Beyoncé will continue to break records and barriers?", \\ 
% "B": "Given her track record, I wouldn't be surprised if she does." \\ 
% "A": "I look forward to seeing her future projects and contributions.", \\ 
% "B": "She's a force to be reckoned with, always pushing boundaries." \\ 
% "A": "Beyoncé's legacy will undoubtedly inspire generations to come.", \\ 
% "B": "Absolutely, her impact on music and culture is unparalleled." \\ 
\textbf{My} \\ 
"A": "I've always been fascinated by Beyoncé's career. Can you tell me more about her achievements and influence in the music industry?", \\ 
"B": "Absolutely, Beyoncé's career is incredibly impressive. She has sold over 118 million records as a solo artist and an additional 60 million with Destiny's Child, solidifying her as one of the best-selling music artists of all time.", \\ 
"A": "I'm curious about her impact on the music industry. Can you elaborate on her influence and recognition?", \\ 
"B": "Certainly, Beyoncé's impact on the music industry is profound. Her dynamic and highly choreographed performances have earned her recognition as one of the best entertainers in contemporary popular music.", \\ 
"A": "I've heard about her numerous awards. Can you provide more details about her accolades and awards?", \\ 
"B": "Absolutely, Beyoncé has received numerous accolades and awards. She has won an impressive 20 Grammy Awards and holds the record for being the most nominated woman in the award's history.", \\ 
"A": "I'm interested in her recognition by industry associations. Can you share more about her industry recognition and achievements?", \\ 
"B": "Certainly, Beyoncé has been widely recognized by industry associations. For instance, the Recording Industry Association of America acknowledged her as the Top Certified Artist in America during the 2000s decade.", \\ 
\dots \\
\noalign{\hrule height 1.5pt}
% \bottomrule
\end{tabular}
\caption{}
\label{tab:case_study_single_column}
\end{table*}
